HiTeA: Hierarchical Temporal-Aware Video-Language Pre-training

Video-language pre-training has advanced the performance of various downstream video-language tasks. However, most previous methods directly inherit or adapt typical image-language pre-training paradigms to video-language pre-training, thus not fully exploiting the unique characteristic of video, i.e., temporal. In this paper, we propose a Hierarchical Temporal-Aware video-language pre-training framework, HiTeA, with two novel pre-training tasks for modeling cross-modal alignment between moments and texts as well as the temporal relations of video-text pairs. Specifically, we propose a cross-modal moment exploration task to explore moments in videos, which results in detailed video moment representation. Besides, the inherent temporal relations are captured by aligning video-text pairs as a whole in different time resolutions with multi-modal temporal relation exploration task. Furthermore, we introduce the shuffling test to evaluate the temporal reliance of datasets and video-language pre-training models. We achieve state-of-the-art results on 15 well-established video-language understanding and generation tasks, especially on temporal-oriented datasets (e.g., SSv2-Template and SSv2-Label) with 8.6% and 11.1% improvement respectively. HiTeA also demonstrates strong generalization ability when directly transferred to downstream tasks in a zero-shot manner. Models and demo will be available on ModelScope.

==> tables/image_retrieval.tex <==
\begin{table*}[t]
\vspace{1em}
\tablestyle{3.5pt}{1.05}
\begin{tabular}{lrcccccccccccc}
\shline
\multirow{3}{*}{ Method } & \multirow{3}{*}{ \#PT } & \multicolumn{6}{c}{COCO (5K test)} & \multicolumn{6}{c}{Flickr30K (1K test)} \\ 
& & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{IR } & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{IR } \\ \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
& & R1 & R5 & R10 & R1 & R5 & R10 & R1 & R5 & R10 & R1 & R5 & R10 \\
\midrule
ViLT~\cite{kim2021vilt} & 4M & 61.5 & 86.3 & 92.7 & 42.7 & 72.9 & 83.1 & 83.5 & 96.7 & 98.6 & 64.4 & 88.7 & 93.8 \\
UNITER~\cite{chen2019uniter} & 4M & 65.7 & 88.6 & 93.8 & 52.9 & 79.9 & 88.0 & 87.3 & 98.0 & 99.2 & 75.6 & 94.1 & 96.8 \\
OSCAR~\cite{li2020oscar} & 4M & 70.0 & 91.1 & 95.5 & 54.0 & 80.8 & 88.5 &- &- &- & - & - & - \\
Frozen~\cite{bain2021frozen} & 5M & - &- &- & - & - & - &- &- &- & 61.0 & 87.5 & 92.7 \\
ALBEF~\cite{li2021align} & 4M & 73.1 & 91.4 & 96.0 & 56.8 & 81.5 & 89.2 & 94.3 & 99.4 & 99.8 & 82.8 & 96.7 & 98.4 \\
BLIP~\cite{li2022blip} & 14M & 80.6 & 95.2 & 97.6 & 63.1 & 85.3 & 91.1 & 96.6 & 99.8 & 100.0 & 87.2 & 97.5 & 98.8 \\
ALIGN~\cite{jia2021scaling} & 1.2B & 77.0 & 93.5 & 96.9 & 59.9 & 83.3 & 89.8 & 95.3 & 99.8 & 100.0 & 84.9 & 97.4 & 98.6 \\
Singularity~\cite{lei2022singularity} & 5M & 71.9 & 90.8 & 95.4 & 54.6 & 80.0 & 87.8 & 93.3 & 99.4 & 99.8 & 81.4 & 95.8 & 97.9 \\
\hline
\modelname & 5M & 71.9 & 90.8 & 95.4 & 54.6 & 80.0 & 87.8 & 93.3 & 99.4 & 99.8 & 81.4 & 95.8 & 97.9 \\
\shline
\end{tabular}
\caption{Comparison to existing methods on image-text retrieval. We show results for both text retrieval (image-to-text retrieval, TR) and image retrieval (IR).}
\label{tab:img_ret}
\end{table*}
%%%%%%%%%%%%%
